Improving "Fast Iterative Shrinkage-Thresholding Algorithm": Faster, Smarter and Greedier

The "fast iterative shrinkage-thresholding algorithm", a.k.a. FISTA, is one of the most well-known first-order optimisation scheme in the literature, as it achieves the worst-case $O(1/k^2)$ optimal convergence rate in terms of objective function value. However, despite such an optimal theoretical convergence rate, in practice the (local) oscillatory behaviour of FISTA often damps its efficiency. Over the past years, various efforts are made in the literature to improve the practical performance of FISTA, such as monotone FISTA, restarting FISTA and backtracking strategies. In this paper, we propose a simple yet effective modification to the original FISTA scheme which has two advantages: it allows us to 1) prove the convergence of generated sequence; 2) design a so-called "lazy-start" strategy which can up to an order faster than the original scheme. Moreover, by exploring the properties of FISTA scheme, we propose novel adaptive and greedy strategies which probes the limit of the algorithm. The advantages of the proposed schemes are tested through problems arising from inverse problem, machine learning and signal/image processing.

==> tex/sec-conclusion.tex <==
\section{Discussion and conclusion}\label{sec:conclusion}

In this paper, we proposed a generalized inertial Forward--Backward splitting scheme which covers several existing methods as special cases, and presented the corresponding global convergence analysis.
Under partial smoothness, we established that this class of schemes identify the active manifold in finite time, and then converge locally linearly. The predicted rates were shown to be very sharp.
We verified our theoretical findings with concrete numerical examples from signal/image processing and machine learning.

Most of our results can be extended to the non-convex setting by introducing appropriate supplementary assumptions, such as prox-regularity and the non-smooth Kurdyka-{\L}ojasiewicz inequality. This will be treated in a future work.


